Controlling Graph Dynamics with Reinforcement Learning and Graph Neural Networks

We consider the problem of controlling a partially-observed dynamic process on a graph by a limited number of interventions. This problem naturally arises in contexts such as scheduling virus tests to curb an epidemic; targeted marketing in order to promote a product; and manually inspecting posts to detect fake news spreading on social networks. We formulate this setup as a sequential decision problem over a temporal graph process. In face of an exponential state space, combinatorial action space and partial observability, we design a novel tractable scheme to control dynamical processes on temporal graphs. We successfully apply our approach to two popular problems that fall into our framework: prioritizing which nodes should be tested in order to curb the spread of an epidemic, and influence maximization on a graph.

==> AAAI2021/scratch.tex <==


%Finally, all these systems continuously evolve, whether it is because the underlying temporal network connectivity is altered (e.g, social contacts in an epidemic setup) or because the network properties are modified (e.g., workloads in server farms or interests or trending topics in online social networks).

%\section{Introduction}
%Complex environments can often be modelled as dynamic networks, which  continuously change their activity states and connectivity patterns.  In many cases, it is desirable to intervene with this dynamic and control its outcome. The problem of learning such control interventions is fundamental to artificial intelligence. 
%An important motivating example is the problem of controlling an epidemic which spreads by infecting people across their physical social network. Recent attempts to control COVID-19 suggest that isolating infected individuals can be major factor in slowing and containing the disease. Identifying  infected patients requires to administer tests at large scale, and it becomes critical to prioritize which individuals should be tested and isolated. 

%Controlling diffusive processes over a network is important in many other problems, including phenomana like product adaption, opinions spreading on social network, viruses inflicting computer networks and cascades of failures in server farms. In all these cases, the systems continuously evolve, and   their dynamics  can be manipulated by point interventions on nodes of the network. For example, users of social networks may share information with their immediate neighborhood, and one may be interested to target a small subset of nodes of the social network to clarify or undo the effect of such information.

%For COVID-19, since no cure is available, it is critical to develop methods to curb the exponential growth of the epidemic to a contained growth pattern. Since global quarantines and lock-down carry an immense economical cost,  it is necessary to identify epidemic carriers and isolate them from the population. This poses a major question: How should such point-wise interventions be prioritized to best reduce the contagation spread? 
%This question is an instance of a general phenomena. Diffusive  processes on networks are prevalent in our world, and include phenomana  such product adaption, opinions spreading on social network, viruses inflicting computer networks and cascades of failures in server farms. The dynamics of these processes can be manipulated by point interactions  on the network.
% Infected people can be asked to self-quarantine, preventing the spread of a disease, while computers may be temporarily disconnected or patched by security updates. Users may be shown targeted ads or  articles to promote production adaption or influence their opinion.  Finally, all these systems continuously evolve, whether it is because the underlying temporal network connectivity is altered (e.g, social contacts in an epidemic setup) or because the network properties are modified (e.g., workloads in server farms or interests or trending topics in online social networks).

%\gal{Eli, I suggest the following structure: (1) Par' 1: The problem of decision making over temporal graphs. (2) Par 2' An important example: controlling pandemics  (3) Par 3` two other examples. (4) Par` 4: Straw-men: Why supervised learning is not enough (5) The key ideas of this paper. (6) One  technical contribution.}


%The recent COVID-19 outbreak is expected to cost millions of human lives and billions of dollars. As there is no known cure yet, efforts are dedicated to ``flatten the curve'', i.e, reduce the in-the-wild exponential growth to a contained growth pattern. Strong measures such as quarantining and lock-down are often deployed, with an immense economical impact. \gal{Lets be careful not to make the paper a "Covid-application" paper. It is more general about RL on graphs with propagating activity. }


%The ability to pinpoint and early detect epidemic carriers is the key in order to contain the epidemic for a long period of time in a sustainable manner. However, as the epidemic spreads, the need for test kits grows, and the deficit in testing capacity increases both due to the limited lab capacity and due to logistics constraints, such as obtaining and processing samples from a large portion of the population spread on a vast area on a daily basis. Nevertheless, to curb long infection chains we must identify the epidemic carriers and isolate them from the rest of the population. This poses a major  question: How can we optimize our testing methodology in order to best fight the contagation spread?

%The problem of testing prioritizing in order to minimize the spreading of an epidemic is a specific instance of a general phenomena. Diffusive  processes on networks are prevalent in our world, and include phenomana  such product adaption, opinions spreading on social network, viruses inflicting computer networks and cascades of failures in server farms. The dynamics of these processes can be manipulated by point interactions  on the network. Infected people can be asked to self-quarantine, preventing the spread of a disease, while computers may be temporarily disconnected or patched by security updates. Users may be shown targeted ads or  articles to promote production adaption or influence their opinion.  

%Finally, all these systems continuously evolve, whether it is because the underlying temporal network connectivity is altered (e.g, social contacts in an epidemic setup) or because the network properties are modified (e.g., workloads in server farms or interests or trending topics in online social networks).



\ignore{
    \begin{table*}
    \begin{tabular}{|c|c|c|c|c|}
    \hline 
     & 2 communities & 3 communities & Preferential \\ attachment & contact tracing\tabularnewline
    \hline 
    \hline 
    Tree based model & $0.15\pm0.35$  &  &  & \tabularnewline
    \hline 
    Counter model & $0.19\pm0.39$  &  &  & \tabularnewline
    \hline 
    Supervised (minimal) & $0.24\pm0.11$ & $0.02\pm0.02$ & $0.38\pm0.1$  & $0.05\pm0.05$\tabularnewline
    \hline 
    Supervised (full) & $0.27\pm0.1$  & $0.02\pm0.02$  & $0.76\pm0.1$  & $0.52\pm0.1$\tabularnewline
    \hline 
    Supervised + \\ degree weighted loss & $0.29\pm0.1$  & $0.01\pm0.02$ & $0.77\pm0.09$ & \tabularnewline
    \hline 
    Supervised + class \&  \\ degree weighted loss & $0.24\pm0.1$ & $0.02\pm0.02$  & $0.87\pm0.07$ & \tabularnewline
    \hline 
    RL (minimal) & $0.66\pm0.10$  & $0.07\pm0.05$  & $0.39\pm0.06$ & \tabularnewline
    \hline 
    RL (full) & $\mathbf{0.876\pm0.07}$  & \textbf{$\mathbf{0.53\pm0.13}$ } & \textbf{$\mathbf{0.93\pm0.05}$ } & \textbf{$\mathbf{0.74\pm0.1}$ }\tabularnewline
    \hline 
    \end{tabular}
    \caption{\gal{Keep only communities. Add caption}}
    \label{tab:comaprison-chart}
    \end{table*}
}



%\ignore{
\begin{table}
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.99}{\small{
    \centering
    \begin{tabular}{|l|c|c|}
    \hline 
     & Preferential & contact \\
     & attachment & tracing\\
    \hline 
    \hline 
    Tree based model & $0.20\pm0.02$ & $0.00\pm0.00$ \\
    \hline 
    Counter model & $0.31\pm0.02$ & $0.02\pm0.01$\\
    \hline 
    Supervised (vanilla) & $0.38\pm0.10$ & $0.05\pm0.05$\\
    \hline 
    RL minimal (ours) & $0.39\pm0.06$ & \\
    \hline 
    Supervised +GNN & $0.76\pm0.10$ & $0.52\pm0.1$\\
    \hline 
    Supervised +GNN+deg & $0.77\pm0.09$ & $0.54\pm0.11$\\
    \hline 
    RL full (ours) & \textbf{$0.93\pm0.05$} & \textbf{$0.74\pm0.1$}\\
    \hline 
    \end{tabular}
    }}
\caption{Percentage of epidemics contained, in PA and contact-tracing Comparison across methods on scale-free network models of $200$ nodes. Values are the probability of containing an epidemic in percents $\pm$ is empirical standard deviation.}
\label{tab:comaprison-chart-scale-free}
\end{table}
%}


\begin{table}
\centering
    \setlength{\tabcolsep}{3pt}
    \scalebox{0.99}{\small{\sc{
    \centering
        \begin{tabular}{|l|c|c|c|c|}
        \hline
        & \multicolumn{2}{c}{\%contained} & \multicolumn{2}{c}{\%healthy} \\
        \hline
         & PA & CT & PA & CT\\
        \hline 
        \hline 
        Tree based model  &  & $0\pm0$ &  & $11\pm3$\\
        \hline 
        Counter model &  $ & 0\pm0$ &  & $14\pm5$ \\
        \hline 
        SL (vanilla) & $2\pm2$ & $0\pm0$ & $13\pm3$ & $17\pm1$\\
        \hline 
        SL + GNN & $27\pm6$ & $15\pm4$ & $34\pm3$ & $32\pm$2\\
        \hline 
        SL + deg & $3\pm3$ & $0\pm1$ & $15\pm3$ & $18\pm1$\\
        \hline 
        SL + deg + GNN & $26\pm5$ & $16\pm5$ & $33\pm3$ & $32\pm1$\\
        \hline 
        RL (vanilla) & $2\pm2$ & $1\pm1$ & $17\pm1$ & $16\pm1$\\
        \hline 
        RLGN (ours) & \textbf{$\mathbf{78\pm4}$} & $\mathbf{45\pm6}$ & $\mathbf{52\pm2}$ & $\mathbf{40\pm1}$\\
        \hline 
        \end{tabular}
    }}}
    \caption{Percent of contained epidemics and percent of healthy nodes achieved using all methods on a PA network (n=$200$ nodes), and CT network.}
\label{tab:comaprison-chart-scale-free}
\end{table}
